Tripletformer for Probabilistic Interpolation of Irregularly sampled Time Series

Irregularly sampled time series data with missing values is observed in many fields like healthcare, astronomy, and climate science. Interpolation of these types of time series is crucial for tasks such as root cause analysis and medical diagnosis, as well as for smoothing out irregular or noisy data. To address this challenge, we present a novel encoder-decoder architecture called "Tripletformer" for probabilistic interpolation of irregularly sampled time series with missing values. This attention-based model operates on sets of observations, where each element is composed of a triple of time, channel, and value. The encoder and decoder of the Tripletformer are designed with attention layers and fully connected layers, enabling the model to effectively process the presented set elements. We evaluate the Tripletformer against a range of baselines on multiple real-world and synthetic datasets and show that it produces more accurate and certain interpolations. Results indicate an improvement in negative loglikelihood error by up to 32% on real-world datasets and 85% on synthetic datasets when using the Tripletformer compared to the next best model.

==> apdx2.tex <==
\begin{table}[ht]
	\centering
	\scriptsize
	\caption{Results for AsTS for \textbf{observations missing at random} on real AsTS datasets. Evaluation measure is Mean Squared Error, lower the best. }
	\label{tab:det_random}
	\begin{tabular}{l|c|c|c}
		\toprule
		tp. obs. & $10\%$  & $50\%$ & $90\%$ \\
		\hline
		\multicolumn{4}{c}{Physionet} \\
		\hline
		Mean & 0.976 & 0.971 & 0.963\\
		Forward & 0.891 & 0.655 & 0.548\\
		GPR & 0.586{\tiny $\pm$0.000} & 0.424{\tiny $\pm$0.002} & 0.414{\tiny $\pm$0.000}\\
		L-ODE-RNN & 0.690{\tiny $\pm$0.021}& 0.618{\tiny $\pm$0.047}& 0.718{\tiny $\pm$0.058} \\
		L-ODE-ODE & 0.581{\tiny $\pm$0.001}& 0.493{\tiny $\pm$0.003}& 0.497{\tiny $\pm$0.006} \\
		mTAN & 0.530{\tiny $\pm$0.001} & 0.377{\tiny $\pm$0.001} & 0.368{\tiny $\pm$0.002}\\
		HETVAE	& 0.549{\tiny $\pm$0.001}& 0.378{\tiny $\pm$0.001}& 0.343{\tiny $\pm$0.002}\\
		Tripletformer & \textbf{0.525{\tiny $\pm$0.006}} & \textbf{0.372{\tiny $\pm$0.007}} & \textbf{0.331{\tiny $\pm$0.011}} \\
		\hline
		\multicolumn{4}{c}{MIMIC-III} \\
		\hline
		Mean & 1.198 & 1.194 & 1.210\\
		Forward & 1.893 & 0.984 & 0.792 \\
		GPR & 1.055{\tiny $\pm$0.006} & 0.480{\tiny $\pm$0.010} & 0.425{\tiny $\pm$0.001} \\
		mTAN & 0.661{\tiny $\pm$0.001} & 0.477{\tiny $\pm$0.001} & 0.474{\tiny $\pm$0.001}\\
		HETVAE	& 0.676{\tiny $\pm$0.001} & 0.472{\tiny $\pm$0.001} & 0.430{\tiny $\pm$0.001} \\
		Tripletformer & \textbf{0.646{\tiny $\pm$0.023}} & \textbf{0.462{\tiny $\pm$0.017}} & \textbf{0.414{\tiny $\pm$0.008}} \\
		\hline
		\multicolumn{4}{c}{Physionet2019} \\
		\hline
		Mean & 1.008 & 1.009 & 1.008\\
		Forward & 0.875 & 0.642 & 0.569 \\
		GPR & 0.611{\tiny $\pm$0.001} & 0.406{\tiny $\pm$0.002} & 0.368{\tiny $\pm$0.001} \\
		mTAN & \textbf{0.581{\tiny $\pm$0.002}} & 0.419{\tiny $\pm$0.002} & 0.415{\tiny $\pm$0.005}\\
		HETVAE	& 0.593{\tiny $\pm$0.000} & 0.410{\tiny $\pm$0.001} & \textbf{0.350{\tiny $\pm$0.000}}\\
		Tripletformer & 0.585{\tiny $\pm$0.001} & \textbf{0.392{\tiny $\pm$0.001}} & 0.371{\tiny $\pm$0.003}\\
		\hline
		\multicolumn{4}{c}{PenDigits} \\
		
		\hline
		Mean & 1.010 & 1.002 & 0.943\\
		Forward & 1.296 & 1.508 & 1.425\\
		GPR & 1.372{\tiny $\pm$0.004}& 0.654{\tiny $\pm$0.008} & 0.462{\tiny $\pm$0.012} \\
		L-ODE-RNN & 0.729{\tiny $\pm$0.009}& 0.519{\tiny $\pm$0.024}& 0.356{\tiny $\pm$0.027} \\
		L-ODE-ODE & 0.773{\tiny $\pm$0.001}& 0.515{\tiny $\pm$0.002}& 0.358{\tiny $\pm$0.013} \\
		mTAN & 0.783{\tiny $\pm$0.004}&  0.453{\tiny $\pm$0.007}& 0.335{\tiny $\pm$0.018}\\
		HETVAE & 0.814{\tiny $\pm$0.001}& 0.725{\tiny $\pm$0.019}& 0.848{\tiny $\pm$0.011}\\
		Tripletformer & 0.695{\tiny $\pm$0.008} & \textbf{0.326{\tiny $\pm$0.003}} & 0.215{\tiny $\pm$0.016}\\
		\hline
		
		\multicolumn{4}{c}{PhonemeSpectra} \\
		\hline
		Mean & 1.066 & 1.060 & 1.072\\
		Forward & 1.360 & 1.348 & 1.237\\
		GPR & 0.924{\tiny $\pm$0.003}& 0.793{\tiny $\pm$0.008}& 0.681{\tiny $\pm$0.011} \\
		L-ODE-RNN & 0.812{\tiny $\pm$0.013}& 0.736{\tiny $\pm$0.018}& 0.68{\tiny $\pm$0.051}\\
		L-ODE-ODE & 0.768{\tiny $\pm$0.004}& 0.705{\tiny $\pm$0.012}& 0.684{\tiny $\pm$0.019} \\
		mTAN & 0.698{\tiny $\pm$0.005} & 0.409{\tiny $\pm$0.006} & 0.515{\tiny $\pm$0.016}\\
		HETVAE & 0.785{\tiny$\pm$0.002}& 0.385{\tiny $\pm$0.010}& 0.528{\tiny$\pm$0.004}\\
		Tripletformer & \textbf{0.679{\tiny $\pm$0.011}} & 0.367{\tiny $\pm$0.035} & {\tiny 0.210$\pm$0.009}\\
		\bottomrule
		
	\end{tabular}
\end{table}

\begin{table}[ht]
	\centering
	\scriptsize
	\caption{Results for AsTS for \textbf{bursts of observations missing} on real AsTS datasets. Evaluation measure is Mean Squared Error, lower the best.}
	\label{tab:det_burst}
	\begin{tabular}{l|c|c|c}
		\toprule
		tp. obs. & $10\%$  & $50\%$ & $90\%$ \\
		\hline
		\multicolumn{4}{c}{Physionet} \\
		\hline
		Mean & 0.974 & 0.973 & 0.984\\
		Forward & 1.297 & 0.958 & 0.697\\
		GPR & 0.708{\tiny $\pm$0.025} & 0.593{\tiny $\pm$0.002} & 0.336{\tiny $\pm$0.001} \\
		L-ODE-RNN & 0.697{\tiny $\pm$0.005}& 0.922{\tiny $\pm$0.009}& 0.737{\tiny $\pm$0.023}	 \\
		L-ODE-ODE &0.684{\tiny $\pm$0.000}& 0.639{\tiny $\pm$0.003}& 0.644{\tiny $\pm$0.002}\\
		mTAN & 0.646{\tiny $\pm$0.001} & 0.569{\tiny $\pm$0.002} & 0.392{\tiny $\pm$0.001}\\
		HETVAE	& 0.635$\pm$0.002 & 0.567$\pm$0.002 & \textbf{0.331$\pm$0.001}\\
		Tripletformer & \textbf{0.627{\tiny $\pm$0.001}} & \textbf{0.554{\tiny $\pm$0.004}} & 0.335{\tiny $\pm$0.003}\\
		\hline
		\multicolumn{4}{c}{MIMIC-III} \\
		\hline
		Mean & 1.199 & 1.197 & 1.199\\
		Forward & 2.388 & 1.436 & 0.953 \\
		GPR & 1.164{\tiny $\pm$0.001} & 0.761{\tiny $\pm$0.005} & 0.468{\tiny $\pm$0.040} \\
		mTAN & 0.805{\tiny $\pm$0.001} & 0.710{\tiny $\pm$0.001} & 0.511{\tiny $\pm$0.001}\\
		HETVAE	& 0.804{\tiny $\pm$0.002} & 0.727{\tiny $\pm$0.002}& \textbf{0.446{\tiny $\pm$0.000}}\\
		Tripletformer & \textbf{0.788{\tiny $\pm$0.002}} & \textbf{0.684{\tiny $\pm$0.001}} & 0.448{\tiny $\pm$0.002} \\
		\hline
		\multicolumn{4}{c}{Physionet2019} \\
		\hline
		Mean & 1.008 & 1.010 & 1.004\\
		Forward & 1.107 & 0.916 & 0.672 \\
		GPR & 0.765{\tiny $\pm$0.000} & 0.522{\tiny $\pm$0.000} & 0.476{\tiny $\pm$0.003} \\
		mTAN & 0.737{\tiny $\pm$0.001} & 0.541{\tiny $\pm$0.001} & 0.461{\tiny $\pm$0.002} \\
		HETVAE	& 0.744{\tiny $\pm$0.005} & 0.515{\tiny $\pm$0.000} & 0.485{\tiny $\pm$0.002}\\
		Tripletformer & \textbf{0.591{\tiny $\pm$0.009}} & \textbf{0.392{\tiny $\pm$0.001}} & \textbf{0.370{\tiny $\pm$0.003}}\\
		\hline
		\multicolumn{4}{c}{PenDigits} \\
		
		\hline
		Mean & 1.017 & 0.954& 0.943 \\
		Forward & 1.311 & 1.694 & 1.425\\
		GPR & 1.287{\tiny $\pm$0.002}& 0.846{\tiny $\pm$0.010} & 0.462{\tiny $\pm$0.012}  \\
		L-ODE-RNN & 0.701{\tiny $\pm$0.004}& 0.524{\tiny $\pm$0.01}& 0.356{\tiny $\pm$0.027} \\
		L-ODE-ODE & 0.694{\tiny $\pm$0.002}& 0.568{\tiny $\pm$0.04}& 0.358{\tiny $\pm$0.013} \\
		mTAN & 0.743{\tiny $\pm$0.003} & 0.466{\tiny $\pm$0.005} & 0.335{\tiny $\pm$0.018} \\
		HETVAE & 0.736{\tiny $\pm$0.026}& 0.723{\tiny $\pm$0.001} & 0.848{\tiny $\pm$0.011}\\
		Tripletformer & \textbf{0.644{\tiny $\pm$0.001}} & 0.408{\tiny $\pm$0.004} & \textbf{0.215{\tiny $\pm$0.016}}\\
		\hline
		
		\multicolumn{4}{c}{PhonemeSpectra} \\
		\hline
		Mean & 1.071 & 1.048 & 1.006\\
		Forward & 1.419 & 1.598 & 1.505\\
		GPR & 0.939{\tiny $\pm$0.000}& 0.839{\tiny $\pm$0.000}& 0.799{\tiny $\pm$0.000} \\
		L-ODE-RNN & 0.938{\tiny $\pm$0.019}& 0.873{\tiny $\pm$0.027}& 0.777{\tiny $\pm$0.004} \\
		L-ODE-ODE & 0.894{\tiny $\pm$0.001}& 0.846{\tiny $\pm$0.004} & 0.74{\tiny $\pm$0.002} \\
		mTAN & 0.896{\tiny $\pm$0.001} & \textbf{0.782{\tiny $\pm$0.002}} & 0.817{\tiny $\pm$0.011} \\
		HETVAE & 0.887{\tiny $\pm$0.001} & 0.815{\tiny $\pm$0.001} & 0.808{\tiny $\pm$0.002}\\
		
		Tripletformer & \textbf{0.854$\pm$0.001} & 0.808{\tiny $\pm$0.001} & 0.817{\tiny $\pm$0.00}\\
		\bottomrule
		
	\end{tabular}
\end{table}







\begin{table}[t]
	\centering
	\scriptsize
	\caption{Results of synthetic AsTS for \textbf{observations missing at random}. Evaluation measure is NLL, lower the best. }
	\label{tab:synth:det_random}
	\begin{tabular}{l|c|c|c}
		\toprule
		
		tp. obs. & $10\%$  & $50\%$ & $90\%$ \\
		\hline
		\multicolumn{4}{c}{PenDigits} \\
		
		\hline
		Mean & 1.0103{\tiny $\pm$0.0000} & 1.0027{\tiny $\pm$0.0000} & 0.9437{\tiny $\pm$0.0000}\\
		Forward & 1.2960{\tiny $\pm$0.0000} & 1.5086{\tiny $\pm$0.0000} & 1.4259{\tiny $\pm$0.0000}\\
		GPR & 1.3724{\tiny $\pm$0.0044}& 0.6547{\tiny $\pm$0.0088} & 0.4621{\tiny $\pm$0.0121} \\
		L-ODE-RNN & 0.729{\tiny $\pm$0.009}& 0.519{\tiny $\pm$0.024}& 0.356{\tiny $\pm$0.027} \\
		L-ODE-ODE & 0.1 0.773{\tiny $\pm$0.001}& 0.515{\tiny $\pm$0.002}& 0.358{\tiny $\pm$0.013} \\
		mTAN & 0.7838$\pm$0.0042&  0.4535$\pm$0.0079& 0.3359$\pm$0.0183\\
		HETVAE & 0.8149$\pm$0.0017& 0.7256$\pm$0.0196& 0.8481$\pm$0.0111\\
		Tripletformer & 0.6959$\pm$0.0081 & \textbf{0.326$\pm$0.0035} & 0.2158$\pm$0.0166\\
		\hline
		
		\multicolumn{4}{c}{PhonemeSpectra} \\
		\hline
		Mean & 1.0666{\tiny $\pm$0.0000} & 1.0607{\tiny $\pm$0.0000} & 1.0720{\tiny $\pm$0.0000}\\
		Forward & 1.3601{\tiny $\pm$0.0000} & 1.3488{\tiny $\pm$0.0000} & 1.2372{\tiny $\pm$0.0000}\\
		GPR & 0.9248{\tiny $\pm$0.0038}& 0.7932{\tiny $\pm$0.0089}& 0.6816{\tiny $\pm$0.0116} \\
		L-ODE-RNN & 0.812{\tiny $\pm$0.013}& 0.736{\tiny $\pm$0.018}& 0.68{\tiny $\pm$0.051}\\
		L-ODE-ODE & 0.768{\tiny $\pm$0.004}& 0.705{\tiny $\pm$0.012}& 0.684{\tiny $\pm$0.019} \\
		mTAN & 0.6987{\tiny $\pm$0.0051} & 0.4099{\tiny $\pm$0.0065} & 0.5156{\tiny $\pm$0.0161}\\
		HETVAE & 0.785{\tiny$\pm$0.0020}& 0.3857{\tiny $\pm$0.0102}& 0.5280{\tiny$\pm$0.0040}\\
		Tripletformer & \textbf{0.6792{\tiny $\pm$0.0112}} & 0.3670{\tiny $\pm$0.0359} & {\tiny 0.2106$\pm$0.0091}\\
		\bottomrule
	\end{tabular}
\end{table}


\begin{table}[t]
	\centering
	\scriptsize
	\caption{Results of synthetic AsTS for \textbf{observations missing at burst}. Evaluation measure is NLL, lower the best. }
	\label{tab:synth:det_burst}
	\begin{tabular}{l|c|c|c}
		\toprule
		
		tp. obs. & $10\%$  & $50\%$ & $90\%$ \\
		\hline
		\multicolumn{4}{c}{PenDigits} \\
		
		\hline
		Mean & 1.0179{\tiny $\pm$0.0000} & 0.9542{\tiny $\pm$0.0000} & 0.9437{\tiny $\pm$0.0000} \\
		Forward & 1.3113{\tiny $\pm$0.0000} & 1.6946{\tiny $\pm$0.0000} & 1.4259{\tiny $\pm$0.0000}\\
		GPR & 1.2875{\tiny $\pm$0.0016}& 0.846{\tiny $\pm$0.0101} & 0.4621{\tiny $\pm$0.0121}  \\
		L-ODE-RNN & 0.701{\tiny $\pm$0.004}& 0.524{\tiny $\pm$0.01}& 0.441{\tiny $\pm$0.012} \\
		L-ODE-ODE & 0.694{\tiny $\pm$0.002}& 0.568{\tiny $\pm$0.04}& 0.496{\tiny $\pm$0.148} \\
		mTAN & 0.7435$\pm$0.003& 0.4669$\pm$0.0053 & 0.3359$\pm$0.0183 \\
		HETVAE & 0.7361$\pm$0.0263& 0.7236$\pm$0.0009 & 0.8481$\pm$0.0111\\
		Tripletformer & \textbf{0.6441$\pm$0.0006} & 0.4084$\pm$0.0047 & \textbf{0.2158$\pm$0.0166}\\
		\hline
		
		\multicolumn{4}{c}{PhonemeSpectra} \\
		\hline
		Mean & 1.0713{\tiny $\pm$0.0000} & 1.0486{\tiny $\pm$0.0000} & 1.0067{\tiny $\pm$0.0000}\\
		Forward & 1.4192{\tiny $\pm$0.0000} & 1.5983{\tiny $\pm$0.0000} & 1.5052{\tiny $\pm$0.0000}\\
		GPR & 0.9390$\pm$0.0001& 0.8390$\pm$0.0001& 0.7990$\pm$0.0002 \\
		L-ODE-RNN & 0.938{\tiny $\pm$0.019}& 0.873{\tiny $\pm$0.027}& 0.777{\tiny $\pm$0.004} \\
		L-ODE-ODE & 0.894{\tiny $\pm$0.001}& 0.846{\tiny $\pm$0.004} & 0.74{\tiny $\pm$0.002} \\
		mTAN & 0.8959{\tiny $\pm$0.0013} & \textbf{0.7821{\tiny $\pm$0.0022}} & 0.8174{\tiny $\pm$0.0114} \\
		HETVAE & 0.8874$\pm$0.0005 & 0.8159$\pm$0.0004 & 0.8088$\pm$0.0015\\
		
		Tripletformer & \textbf{0.8542$\pm$0.0006} & 0.8083$\pm$0.001 & 0.8172$\pm$0.0026\\
		\bottomrule
		
	\end{tabular}
\end{table}








%\newpage
%
%
%\begin{table*}[t]
%	\centering
%	\scriptsize
%	\caption{Results for AsTS for \textbf{observations missing at random} on real AsTS datasets. Evaluation measure is NLL, lower the best. }
%	\label{tab:random_none}
%	\begin{tabular}{l|l|c|c|c|c|c|c|}
%		\toprule
%	&	tp. obs. & \multicolumn{2}{c|}{$10\%$}  & \multicolumn{2}{c|}{$50\%$} & \multicolumn{2}{c|}{$90\%$} \\
%	\cline{3-4} \cline{5-6} \cline{7-8}
%	&	Samp. tech. & NLL & MSE & NLL & MSE & NLL & MSE \\
%		\hline
%		\multirow{6}{*}{Physionet2012}
%	&	Mean & 1.4069{\tiny $\pm$0.0000} & & 1.4067{\tiny $\pm$0.0000} & & 1.4020{\tiny $\pm$0.0000} & \\
%	&	Forward & 1.3719{\tiny $\pm$0.0000} & & 1.2175{\tiny $\pm$0.0000} & & 1.1646{\tiny $\pm$0.0000} &\\
%	&	GPR & 0.9560{\tiny $\pm$0.0005} & 0.5867{\tiny $\pm$0.0001} & 0.7671{\tiny $\pm$0.0060} & 0.4241{\tiny $\pm$0.0017} & 0.7986{\tiny $\pm$0.0043} & 0.4146{\tiny $\pm$0.0002} \\
%	&	mTAN & 1.1107{\tiny $\pm$0.0005} & & 0.9341{\tiny $\pm$0.0014} & & 0.9238{\tiny $\pm$0.0020} &\\
%	&	HETVAE	& 0.8492{\tiny $\pm$0.0082} & 0.4146{\tiny $\pm$0.0002}	& 0.5785{\tiny $\pm$0.0057}	& 0.3786$\pm$0.0006 &	0.5510{\tiny $\pm$0.0119} & 0.3425$\pm$0.002 \\
%	&	Tripletformer & \textbf{0.7804$\pm${\tiny 0.0130}} & & \textbf{0.4551{\tiny $\pm$0.0112}} & & \textbf{0.3734{\tiny $\pm$0.0407}} &\\
%		\hline
%%		\multicolumn{7}{c}{MIMIC-III} \\
%		\hline
%		\multirow{6}{*}{MIMIC-III}
%	&	Mean & 1.5089{\tiny $\pm$0.0000} & & 1.5083{\tiny $\pm$0.0000} & &{\tiny 1.5078$\pm$0.0000}&\\
%	&	Forward & 1.7508{\tiny $\pm$0.0000} & & 1.4236{\tiny $\pm$0.0000} & &{\tiny 1.3283$\pm$0.0000}& \\
%	&	GPR & 0.2012{\tiny $\pm$0.0033} & 1.0554{\tiny$\pm$0.0064} & 0.9797{\tiny $\pm$0.0066} & 0.4806{\tiny$\pm$0.0108} &  0.9192{\tiny $\pm$0.0002} & 0.4255{\tiny$\pm$0.0003}\\
%	&	mTAN & 1.2098{\tiny $\pm$0.0009} & & 1.0665{\tiny $\pm$0.0011} & & 1.0654{\tiny $\pm$0.0019} &\\
%	&	HETVAE	& 1.0778{\tiny $\pm$0.0030}	& 0.6764{\tiny$\pm$0.0014} & 0.8280{\tiny $\pm$0.0012} & 0.4725{\tiny$\pm$0.0005}	&	0.7748{\tiny $\pm$0.0086} & 0.4307{\tiny$\pm$0.0013} \\
%	&	Tripletformer & \textbf{1.0562{\tiny $\pm$0.0067}} & & \textbf{0.7890{\tiny $\pm$0.0064}} & & \textbf{0.7106{\tiny $\pm$0.0105}} & \\
%		\hline
%%		\multicolumn{7}{c}{Physionet2019} \\
%		\hline
%		\multirow{6}{*}{Physionet2019}
%	&	Mean & 1.4210{\tiny $\pm$0.0000} && 1.4207{\tiny $\pm$0.0000} &&1.4252{\tiny $\pm$0.0000}&\\
%	&	Forward & 1.3617{\tiny $\pm$0.0000} && 1.2053{\tiny $\pm$0.0000} && 1.4333{\tiny $\pm$0.0000}&  \\
%	&	GPR & 1.1366{\tiny $\pm$0.0003} & 0.6114{\tiny$\pm$0.0004} &  0.9070{\tiny $\pm$0.0128} & 0.4063{\tiny$\pm$0.0027} & 0.8516{\tiny $\pm$0.0078}& 0.3685{\tiny$\pm$0.0005} \\
%	&	mTAN &  1.1523{\tiny $\pm$0.0011} && 0.9889{\tiny $\pm$0.0029} && 0.9829{\tiny $\pm$0.0068}&\\
%	&	HETVAE	& 1.0917{\tiny $\pm$0.0005}& 0.3498{\tiny$\pm$0.0004} & 0.8555{\tiny $\pm$0.0022} & 0.41{\tiny$\pm$0.0006} & 0.8350{\tiny $\pm$0.0053}& 0.3498{\tiny$\pm$0.0004}\\
%	&	Tripletformer & \textbf{1.0795{\tiny $\pm$0.0016}}& &\textbf{0.8060{\tiny $\pm$0.0040}} & & \textbf{0.7523{\tiny $\pm$0.0070}}&\\
%		\bottomrule
%		
%	\end{tabular}
%\end{table*}
%
%
%
%
%
%
%
%\begin{table*}[t]
%	\centering
%	\scriptsize
%	\caption{Results for AsTS for \textbf{bursts of observations missing} on real AsTS datasets. Evaluation measure is NLL, lower the best.}
%	\label{tab:burst}
%	\begin{tabular}{l|l|c|c|c|c|c|c|}
%		
%		\toprule
%&	tp. obs. & \multicolumn{2}{c|}{$10\%$}  & \multicolumn{2}{c|}{$50\%$} & \multicolumn{2}{c|}{$90\%$} \\
%\cline{3-4} \cline{5-6} \cline{7-8}
%&	Samp. tech. & NLL & MSE & NLL & MSE & NLL & MSE \\
%\hline
%		\multirow{6}{*}{Physionet2012}	
%	&	Mean & 1.4121{\tiny $\pm$0.0000} & & 1.3822{\tiny $\pm$0.0000}& & 1.4069{\tiny $\pm$}0.0000 &\\
%	&	Forward & 1.5345{\tiny $\pm$0.0000}& &1.4424{\tiny $\pm$0.0000} & &1.2327{\tiny $\pm$0.0000} &\\
%	&	GPR & 1.1275{\tiny $\pm$0.0184} & 0.7087{\tiny $\pm$0.0258} & 0.9833{\tiny $\pm$0.0026} & 0.5932{\tiny $\pm$0.0018} & 0.6915{\tiny $\pm$0.0018} & 0.3363{\tiny $\pm$0.0003} \\
%	&	mTAN & 1.2005{\tiny $\pm$0.0003} & & 1.1413{\tiny $\pm$0.0016} & & 0.9605{\tiny $\pm$0.0019} &\\
%	&	HETVAE	& 1.0280{\tiny $\pm$0.0116} & 0.6358{\tiny $\pm$0.002} & 0.8823{\tiny $\pm$0.0026} & 0.5673{\tiny $\pm$0.0014} & 0.6145{\tiny $\pm$0.0394} & \textbf{0.3316{\tiny $\pm$0.0012}}\\
%	&	Tripletformer & \textbf{0.9254{\tiny $\pm$0.0057}}& \textbf{0.6275{\tiny $\pm$0.0014}} & \textbf{0.7770{\tiny $\pm$0.0135}} & \textbf{0.5542{\tiny $\pm$0.0039}} & \textbf{0.5782{\tiny $\pm$0.0345}}  & 0.3349{\tiny $\pm$0.0035}\\
%		\hline
%		\hline
%		\multirow{6}{*}{MIMIC-III}
%	&	Mean & 1.5093{\tiny $\pm$0.0000} & & 1.5076{\tiny $\pm$0.0000} & & 1.5155{\tiny $\pm$0.0000} &\\
%	&	Forward & 1.8709{\tiny $\pm$0.0000} & & 1.6083{\tiny $\pm$0.0000} & &1.4127{\tiny $\pm$0.0000} &\\
%	&	GPR & 1.3286{\tiny $\pm$0.0002} & 1.1648{\tiny $\pm$0.0003} & 1.2319{\tiny $\pm$0.0043}& 0.7613{\tiny $\pm$0.005} & 1.0007{\tiny $\pm$0.0398} & 0.4688{\tiny $\pm$0.0403} \\
%	&	mTAN & 1.3192{\tiny $\pm$0.0006} & & 1.2474{\tiny $\pm$0.0008} & & 1.0949{\tiny $\pm$0.0006} &\\
%	&	HETVAE	& 1.2105{\tiny $\pm$0.0008} & 0.804{\tiny $\pm$0.0018} & 1.1262{\tiny $\pm$0.0033}  & 0.7271{\tiny $\pm$0.0025} & 0.9399{\tiny $\pm$0.0093} & \textbf{0.4462{\tiny $\pm$0.0003}}\\
%	&	Tripletformer & \textbf{1.1938{\tiny $\pm$0.0034}} & \textbf{0.7883{\tiny $\pm$0.0019}} & \textbf{1.0878{\tiny $\pm$0.0062}} & \textbf{0.6842{\tiny $\pm$0.0006}} &  \textbf{0.8854{\tiny $\pm$0.0321}} & 0.4484{\tiny $\pm$0.0017}\\
%		\hline
%		\hline
%		\multirow{6}{*}{Physionet2019}
%	&	Mean & 1.4250{\tiny $\pm$0.0000} & & 1.4159{\tiny $\pm$0.0000}& &1.4195{\tiny $\pm$0.0000}&\\
%	&	Forward & 1.4666{\tiny $\pm$0.0000} && 1.3684{\tiny $\pm$0.0000} & & 1.2097{\tiny $\pm$0.0000} &\\
%	&	GPR & 0.8586{\tiny $\pm$0.0000} & 0.7651{\tiny $\pm$0.0001} & 1.0491{\tiny $\pm$0.0022} & 0.5224{\tiny $\pm$0.0004} & 0.9757{\tiny $\pm$0.0053} & 0.476{\tiny $\pm$0.0032} \\
%	&	mTAN & 1.2698{\tiny $\pm$0.0005} & & 1.1138{\tiny $\pm$0.0006} & & 1.0425{\tiny $\pm$0.0027} &\\
%	&	HETVAE	& 1.2417{\tiny $\pm$0.0017}& 0.7444{\tiny $\pm$0.0053} & 1.0126{\tiny $\pm$0.0047} & 0.5156{\tiny $\pm$0.0003} & 0.9497{\tiny $\pm$0.0028} &0.4855{\tiny $\pm$0.0025}\\
%	&	Tripletformer & \textbf{1.2221{\tiny $\pm$0.0011}}&\textbf{0.5913{\tiny $\pm$0.0092}} &  \textbf{0.9778{\tiny $\pm$0.0055}} & \textbf{0.3921{\tiny $\pm$0.0005}} & \textbf{0.8659{\tiny $\pm$0.0091}} & \textbf{0.3705{\tiny $\pm$0.0028}} \\
%		\bottomrule
%		
%	\end{tabular}
%\end{table*}





%\section{Experiment using the Physionet2012 data setup used in~\cite{SM22}}
%\label{apdx:exp_physio}
%
%\begin{table}[ht]
%	\scriptsize
%	\caption{Comparing Tripletformer with competing models using the data setup provided in~\cite{SM22}. Main evaluation metric is NLL and additional metrics used are Mean Absolute Error (MAE), and Mean Squared Error (MSE). Lower the best.}
%	\label{tab:physio_hetvae_setup}
%\begin{tabular}{lccc}
%	\hline
%	 Model & NLL & MAE & MSE \\
%	\hline
%	Mean & $-$ & $0.7396 \pm 0.0000$ & $1.1634 \pm 0.0000$ \\
%	Forward & $-$ & $0.4840 \pm 0.0000$ & $0.9675 \pm 0.0000$ \\
%	GPR & $0.7875 \pm 0.0005$ & $0.4075 \pm 0.0001$ & $0.6110 \pm 0.0003$ \\
%%	Multi-Task GP & $0.9250 \pm 0.0040$ & $0.4178 \pm 0.0007$ & $0.7381 \pm 0.0051$ \\
%%	HVAE RNN & $1.5220 \pm 0.0019$ & $0.7634 \pm 0.0014$ & $1.2061 \pm 0.0038$ \\
%%	HVAE RNN-ODE & $1.4946 \pm 0.0025$ & $0.7372 \pm 0.0026$ & $1.1545 \pm 0.0058$ \\
%%	HVAE ODE-RNN-ODE & $1.2906 \pm 0.0019$ & $0.5334 \pm 0.0020$ & $0.7622 \pm 0.0027$ \\
%	mTAN & $1.2426 \pm 0.0028$ & $0.5056 \pm 0.0004$ & $0.7167 \pm 0.0016$ \\
%	HeTVAE & ${0 . 5 5 4 2} \pm {0 . 0 2 0 9}$ & ${0 . 3 9 1 1} \pm{0 . 0 0 0 4}$ & ${0 . 5 7 7 8} \pm {0 . 0 0 2 0}$ \\
%	\hline
%	Tripleformer & $\mathbf{0.4461 \pm 0.0800}$ & $\mathbf{0.3805 \pm 0.0084}$ & $\mathbf{0.3776 \pm 0.0113}$ \\
%	\hline
%\end{tabular}
%
%\end{table}

==> fig_vis.tex <==
%\begin{figure*}
%	
%	\centering
%	
%	\subfigure{
%	\begin{tikzpicture} 
%	\begin{axis}[%
%	hide axis,
%	xmin=10,
%	xmax=80,
%	ymin=0,
%	ymax=0.4,
%	legend columns=-1,
%	style={column sep=5mm}
%	]
%	\addlegendimage{only marks,mark options=black}
%	\addlegendentry{Observed data};
%	\addlegendimage{only marks,mark options=magenta}
%	\addlegendentry{True Target data};
%	\addlegendimage{blue};
%	\addlegendentry{Tripletformer};
%	\addlegendimage{red};
%	\addlegendentry{HETVAE}
%	\end{axis}
%	\end{tikzpicture}
%}
% \\
%\vspace{-5cm}
%
%\foreach \n in {0,1,2,3,4,5,9,43}
%{
%\subfigure{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/random/0.5/\n.pdf}
%}
%\subfigure{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/bursts/0.5/\n.pdf}
%}
%\hspace{1cm}
%}
%\hspace{-1.3cm}
%
%\setcounter{subfigure}{0}
%\subfigure[][random]{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/random/0.5/48.pdf}
%}
%\subfigure[][bursts]{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/bursts/0.5/48.pdf}
%}
%\setcounter{subfigure}{0}
%\hspace{1cm}
%\subfigure[random]{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/random/0.5/52.pdf}
%}
%\subfigure[bursts]{
%	\includegraphics[width=0.2\linewidth, clip]{fig/quality/physionet/bursts/0.5/52.pdf}
%}
%\end{figure*}



\begin{figure*}
	
	\centering

		\begin{tikzpicture} 
		\begin{axis}[%
		hide axis,
		xmin=10,
		xmax=80,
		ymin=0,
		ymax=0.4,
		legend columns=-1,
		style={draw=none, column sep=5mm}
		]
		\addlegendimage{only marks,mark options=black}
		\addlegendentry{Observed data};
		\addlegendimage{only marks,mark options=magenta}
		\addlegendentry{True Target data};
		\addlegendimage{blue};
		\addlegendentry{Tripletformer};
		\addlegendimage{red};
		\addlegendentry{HETVAE}
		\end{axis}
		\end{tikzpicture}
		
	\vspace{-5cm}
	\begin{subfigure}{\linewidth}
		
	\foreach \n in {0,1,2,3,4,5,9,43}
	{
		\begin{subfigure}{0.2\linewidth}
			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/physionet/random/0.5/\n.pdf}
		\end{subfigure}
		\begin{subfigure}{0.2\linewidth}
			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/physionet/bursts/0.5/\n.pdf}
		\end{subfigure}
		\hspace{1cm}
	}
	\hspace{-1.3cm}
	\begin{subfigure}{0.2\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{fig/quality/physionet/random/0.5/48.pdf}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{fig/quality/physionet/bursts/0.5/48.pdf}
	\end{subfigure}
	\hspace{2.35cm}
	\begin{subfigure}{0.2\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{fig/quality/physionet/random/0.5/52.pdf}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{fig/quality/physionet/bursts/0.5/52.pdf}
	\end{subfigure}

	\caption{\centering Physionet dataset}
	\end{subfigure}

	\begin{subfigure}{\linewidth}
	
	\foreach \n in {6,9,20,26,29,31,51,110}
	{
		\begin{subfigure}{0.2\linewidth}
%			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/mimiciii/random/0.5/\n.pdf}
		\end{subfigure}
		\begin{subfigure}{0.2\linewidth}
%			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/mimiciii/bursts/0.5/\n.pdf}
		\end{subfigure}
		\hspace{1cm}
	}
	\hspace{-1.3cm}
	\begin{subfigure}{0.2\linewidth}

		\includegraphics[width=1\linewidth]{fig/quality/mimiciii/random/0.5/128.pdf}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}

		\includegraphics[width=1\linewidth]{fig/quality/mimiciii/bursts/0.5/128.pdf}
	\end{subfigure}
	\hspace{2.35cm}
	\begin{subfigure}{0.2\linewidth}

		\includegraphics[width=1\linewidth]{fig/quality/mimiciii/random/0.5/169.pdf}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}

		\includegraphics[width=1\linewidth]{fig/quality/mimiciii/bursts/0.5/169.pdf}
	\end{subfigure}
	
	\caption{\centering MIMIC-III dataset}
\end{subfigure}


	\begin{subfigure}{\linewidth}
	
	\foreach \n in {0,1,2,4,7,10,19,21}
	{
		\begin{subfigure}{0.2\linewidth}
			%			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/physionet2019/random/0.5/\n.pdf}
		\end{subfigure}
		\begin{subfigure}{0.2\linewidth}
			%			\centering
			\includegraphics[width=1\linewidth, clip]{fig/quality/physionet2019/bursts/0.5/\n.pdf}
		\end{subfigure}
		\hspace{1cm}
	}
	\hspace{-1.3cm}
	\begin{subfigure}{0.2\linewidth}
		
		\includegraphics[width=1\linewidth]{fig/quality/physionet2019/random/0.5/24.pdf}
		\caption*{\centering random}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}
		
		\includegraphics[width=1\linewidth]{fig/quality/physionet2019/bursts/0.5/24.pdf}
		\caption*{\centering bursts}
	\end{subfigure}
	\hspace{2.35cm}
	\begin{subfigure}{0.2\linewidth}
		
		\includegraphics[width=1\linewidth]{fig/quality/physionet2019/random/0.5/86.pdf}
		\caption*{\centering random}
	\end{subfigure}
	\hspace{3.4mm}
	\begin{subfigure}{0.2\linewidth}
		
		\includegraphics[width=1\linewidth]{fig/quality/physionet2019/bursts/0.5/86.pdf}
		\caption*{\centering bursts}
	\end{subfigure}
	
	\caption{\centering Physionet2019 dataset}
\end{subfigure}
\caption{Visualizations of real-world AsTS datasets. Plots are the predictions (95$^{th}$ percentile) of HETVAE and Tripletformer for heart rate conditioned upon $50\%$ of observations.}
\label{fig:abl_viz}
\end{figure*}
